A model-independent tripartite test of cosmic distance relations

Cosmological distances are fundamental observables in cosmology. The luminosity ($D_L$), angular diameter ($D_A$) and gravitational wave ($D_{\rm GW}$) distances are all trivially related in General Relativity assuming no significant absorption of photons in the extragalactic medium, also known as cosmic opacity. Supernovae have long been the main cosmological standard candle, but bright standard sirens are now a proven alternative, with the advantage of not requiring calibration with other astrophysical sources. Moreover, they can also measure deviations from modified gravity through discrepancies between $D_L$ and $D_{\rm GW}$. However, both gravitational and cosmological parameters are degenerate in the Hubble diagram, making it hard to properly detect beyond standard model physics. Finally, recently a model-independent method named FreePower was proposed to infer angular diameter distances from large-scale structure which is independent of the knowledge of both early universe and dark energy physics. In this paper we propose a tripartite test of the ratios of these three distances with minimal amount of assumptions regarding cosmology, the early universe, cosmic opacity and modified gravity. We proceed to forecast this test with a combination of LSST and Roman supernovae, Einstein Telescope bright sirens and a joint DESI-like + Euclid-like galaxy survey. We find that even in this very model-independent approach we will be able to detect, in each of many redshift bins, percent-level deviations in these ratios of distances, allowing for very precise consistency checks of $\Lambda$CDM and standard physics. It can also result in sub-percent measurements of $H_0$.

==> commented-out.tex <==
%\isa{[ISA: Correct this]} Moreover, we notice that, since $\alpha_M$ is the derivative of $\ln M_*^2$, for the measurement of $\alpha_M$ the constant factor $\lambda$ cancels out, and it can be measured directly with less assumptions. 

%\begin{equation}
%	\sigma\big(\alpha_M(z_i)\big) =  2\frac{\big(1+z_i+ (1/2)\Delta z\big)}{\Delta z} \sqrt{\sigma _{G,i}^2 +\sigma _{G,i+1}^2 +\sigma _{L,i}^2 +\sigma _{L,i+1}^2 }\,. \label{alpha_M}
%\end{equation}


\begin{comment}
\begin{itemize}
	\item No cosmic opacity
\end{itemize}

In this case, $\eta = 0$ and the data values $y_i$ are scattered around  $\lambda^{-1}$. The likelihood is given by:
\begin{equation}
	P(\zeta_i|{\bf x}, {\bf y}) = \int d\lambda \int \left[\prod_{j \neq i}d\zeta_j\right]\exp\left[- \chi_{\bf y}^2(\lambda^{-1}) - \sum_{j=1}^N \chi_{x_j}^2( \Xi_j)\right]\,. \label{prob_Xi}
\end{equation}
Therefore, $\lambda$ will be measured from the contributions of the data points ${\bf y}$ in the first term, and then $\Xi$ will be determined in all redshift bins from ${\bf x}$.

Since $\Xi$ is a ratio of directly measurable variables, if the distances are assumed to have Gaussian errors, then $\Xi$ has a tricky distribution with undefined mean and variance. However, this is not physical, as the errors on distance cannot be exactly Gaussian, otherwise e.g. negative distances would not be impossible. In any case, instead of computing the $\chi^2$ in eq. (\ref{prob_Xi}) exactly, we will use simple propagation of uncertainties here:
\begin{align}
	\left(\frac{\sigma \lambda}{\lambda}\right)^2 & =  \left[\sum_{i=1}^N \left(\sigma_{L,i}^2 + \sigma_{A,i}^2\right)^{-1}\right]^{-1} \,, \\ \left(\frac{\sigma \Xi_i}{\Xi_i}\right)^2 & = \left(\frac{\sigma \lambda}{\lambda}\right)^2 + \sigma _{G,i}^2 + \sigma _{L,i}^2\,, \label{error_Xi}
\end{align}
where $\sigma_{L,i}$, $\sigma_{A,i}$ and $\sigma_{G,i}$ are the relative errors for $D_{L}/\lambda$, $D_A$ and $D_{\rm GW}$ at $z_i$, respectively.

Moreover, we notice that, since $\alpha_M$ is the derivative of $\ln M_*^2$, for the measurement of $\alpha_M$ the constant factor $\lambda$ cancels out, and it can be measured directly. To wit:
%\textcolor{blue}{(LA  I think is better to write everything in explicit terms of errors on $D_{\rm GW}$ and $D_L$ separately, rather than using $\Xi$)}
\begin{equation}
	\sigma\big(\alpha_M(z_i)\big) =  2\frac{\big(1+z_i+ (1/2)\Delta z\big)}{\Delta z} \sqrt{\sigma _{G,i}^2 +\sigma _{G,i+1}^2 +\sigma _{L,i}^2 +\sigma _{L,i+1}^2 }\,. \label{alpha_M}
\end{equation}

%\begin{equation}
%    \sigma\big(\alpha_M(z_i)\big) =  2\frac{\big(1+z_i+ (1/2)\Delta z\big)}{\Delta z} \sqrt{\left(\frac{\sigma \Xi_i}{\isa{\Xi_i}}\right)^2 + \left(\frac{\sigma \Xi_{i+1}}{\isa{\Xi_{i+1}}}\right)^2}\,.
%\end{equation}

\begin{itemize}
	\item All distances coincide when $z \rightarrow 0$
\end{itemize}

A second option is to assume that $\Xi, \eta \rightarrow 1$ at $z \rightarrow 0$, that is, all distances coincide at low redshifts. This is reasonable, since we expect that both cosmic opacity and MG should be integrated effects that accumulate over a range of redshifts -- in the MG framework of section \ref{subsec:Modified_GW}, this equality always holds.

In this case we get rid of $\lambda$ using the first bin, by fixing $ \eta_1 = 1$. The error in this approximation from the MG side ($\Xi_{\text{MG}}$) is $\sim \alpha_{M0}z_1$, which is likely small if we have data at very low redshifts and the modifications of gravity are not that big (see Table~\ref{tab:alpha_M}). The posterior in this case becomes
\begin{align}
	P(\Xi_i, \eta_j|{\bf x}, {\bf y}) = & \int d\lambda \int \left[\prod_{k \neq 1,i}d\Xi_k\right]\left[\prod_{k \neq 1,j}d\eta_k\right] \times \\ & \times\exp\left\{- \chi_{y_1}^2(\lambda^{-1}) - \chi_{x_1}^2(\lambda) - \sum_{k=2}^N \left[\chi_{y_k}^2(\eta_k/\lambda) + \chi_{x_k}^2(\lambda \Xi_k)\right]\right\}\,, \label{prob_Xi_Gamma}
\end{align}
where $\lambda$ is now constrained by the $\chi^2$ of the first bin.

Again, we will approximate the above distribution and simply do propagation of uncertainties, which results in:
\begin{align}
	\left(\frac{\sigma \lambda}{\lambda}\right)^2  & = \left[\left(\sigma_{L,1}^2 + \sigma_{A,1}^2\right)^{-1} + \left(\sigma_{G,1}^2 + \sigma_{L,1}^2\right)^{-1}\right]^{-1} \,, \\
	\left(\frac{\sigma \eta_i}{\eta_i}\right)^2 & = \left(\frac{\sigma \lambda}{\lambda}\right)^2 + \sigma_{L,i}^2 + \sigma_{A,i}^2 \quad (i \neq 1)\,,
\end{align}
while the error in $\Xi_i$ is still given by eq. (\ref{error_Xi}). Finally, the contribution to $\Xi$ containing only the effect of MG ($\Xi_{\text{MG}}$) can be assessed by comparing $D_{\rm GW}$ to $D_A$ directly, and thus the errors in $\alpha_M$ will now be given by eq. (\ref{alpha_M}) with the exchange $\sigma_{L} \rightarrow \sigma_{A}$.
\end{comment}

\begin{comment}
\mq{PRELIMINARY RESULTS USING ONLY DISTANCE DATA}

\begin{figure}
    \includegraphics[width=.49\columnwidth]{figures/error-ratio-LSST01.pdf}\;\;
    \includegraphics[width=.47\columnwidth]{figures/error-alphaM-LSST01.pdf}
    \includegraphics[width=.49\columnwidth]{figures/error-ratio-LSST05.pdf}\;\;\;\;
    \includegraphics[width=.47\columnwidth]{figures/error-alphaM-LSST05.pdf}    
    \caption{
    \mq{
    Forecasts for the errors in $\lambda \,\Xi$ and in $\alpha_M$. Open (closed) markers use redshift bins of width $\Delta z = 0.02$ (0.05). Top (bottom) row assumes a follow-up survey using 10\%  (50\%) of the VRO telescope time. Because $\alpha_M$ is the error in the derivative, it is more sensitive to $\Delta z$. For $\Delta z = 0.05$,  $\sigma (\alpha_M) \simeq 0.2$  can be achieved for the first 6 bins.
    }
    \label{fig:ratio}}
\end{figure}

\begin{figure}
    \centering
    \includegraphics[width=.49\columnwidth]{figures/error-DL-LSST01.pdf} \;\;
    \includegraphics[width=.48\columnwidth]{figures/error-DL-LSST05.pdf} \;\;
    \includegraphics[width=.49\columnwidth]{figures/error-logDL-LSST01.pdf} \;\;
    \includegraphics[width=.48\columnwidth]{figures/error-logDL-LSST05.pdf}
    \caption{
    \mq{
    Forecasts effective errors of $D_L$ in bins for both SN Ia and bright standard sirens. We assume redshift bins of width $\Delta z = 0.05$, and that systematic errors are neglible, so that $\sigma(D_L)^{\rm eff}$ = $\sigma(D_L) / \sqrt{N_{\rm candles}}$. Left (right) panel assumes a follow-up survey using 10\%  (50\%) of the VRO telescope time. Bottom: same for the relative distance errors.
    }
    \label{fig:sigma-DL}}
\end{figure}

\begin{figure}
    \centering
    \includegraphics[width=.5\columnwidth]{figures/hist-LSST01-05.pdf}
    \caption{
    \mq{
    Histogram for the BNS follow-up surveys using 10\% and 50\% of the VRO telescope time.
    }
    \label{fig:histogram}}
\end{figure}

\mq{For the standard sirens, we follow Alfradique 2022 and take forecast for 5 years of the Einstein Telescope, a third-generation gravitational wave observatory, with a very large follow-up program consisting of 50\% of the Vera Rubin Observatory telescope time.}

\mq{Figures~\ref{fig:ratio} and~\ref{fig:sigma-DL} ...}

\isa{Indeed the inclusion of events with gamma-ray bursts (GRB) can only add information in redshifts where we do not have kilonova data, $z \gtrsim 0.5$, since they are much less numerous below that (see Figure~\ref{fig:GWs_GRBs_distribution}). The right panel of figure \ref{fig:GWs_GRBs} shows that we can have a $4-10\%$ relative error in $D_{\rm GW}$ with those events, for a hundred joint detections in total and bin size $dz = 0.05$.}

\begin{figure}
    \centering
    \includegraphics[scale=0.45]{figures/GWs_GRBs_redshift_distribution_dz_0.05.pdf}
    \caption{Number of joint GW and GRB detections per redshift bin, of size $dz = 0.05$.}
    \label{fig:GWs_GRBs_distribution}
\end{figure}

\begin{figure}
    \centering
    \includegraphics[scale=0.45]{figures/GWs_GRBs_sigma_dgw_dz_0.05.pdf}
    \includegraphics[scale=0.45]{figures/GWs_GRBs_sigma_lndgw_dz_0.05.pdf}
    \caption{\isa{Errors in the GW distance in each redshift bin. The detections of GWs with the Einstein Telescope were modelled as in (Matos et al. 2021) but with SNR cutoff equals 12 and merger rate as in (Alfradique et al. 2022). The electromagnetic selection is the same as in (Belgacem et al. 2019), but assuming a hundred joint detections in total.}}
    \label{fig:GWs_GRBs}
\end{figure}

\end{comment}
